Towards a Decentralised Application-Centric Orchestration Framework in the Cloud-Edge Continuum

The efficient management of complex distributed applications in the Cloud-Edge continuum, including their deployment on heterogeneous computing resources and run-time operations, presents significant challenges. Resource management solutions -- also called orchestrators -- play a pivotal role by automating and managing tasks such as resource discovery, optimisation, application deployment, and lifecycle management, whilst ensuring the desired system performance. This paper introduces Swarmchestrate, a decentralised, application-centric orchestration framework inspired by the self-organising principles of Swarms. Swarmchestrate addresses the end-to-end management of distributed applications, from submission to optimal resource allocation across cloud and edge providers, as well as dynamic reconfiguration. Our initial findings include the implementation of the application deployment phase within a Cloud-Edge simulation environment, demonstrating the potential of Swarmchestrate. The results offer valuable insight into the coordination of resource offerings between various providers and optimised resource allocation, providing a foundation for designing scalable and efficient infrastructures.

==> evaluation_copy.tex <==
\section{Evaluation}\label{sec:evaluation}
In this work, we chose the DISSECT-CF-Fog discrete event simulator \cite{markus_2024} as the first testbed to measure and evaluate the effectiveness of the proposed conceptual framework, due to its high realism and customizability in simulating fog computing environments. However, in parallel with the simulator extension, the implementation of the decentralised orchestrator is also underway, supported by the valuable feedback from the simulation tool. DISSECT-CF-Fog enables realistic modelling of physical machines and virtual resources, including their associated energy consumption and network models. Thus, the tool was further enhanced to fully support the conceptualised decentralised approach by integrating the resource agent logic. The results and the implementation are open source and available on GitHub \cite{dissect-cf-fog}.

\subsection{Application submission and offer selection} 

\renewcommand{\arraystretch}{1.25}
\begin{table}[ht]
\centering
\caption{Parameters used for the simulation evaluation}
\label{tab:params}
\resizebox{\linewidth}{!}{
\begin{tabular}{|cc|cc}
\hline
\multicolumn{2}{|c|}{Node}                                              & \multicolumn{2}{c|}{Application}                                    \\ \hline\hline
\multicolumn{1}{|c|}{Location}                            & EU, US      & \multicolumn{1}{c|}{No. of Compute / Storage Type} & \multicolumn{1}{c|}{3 / 1} \\ \hline
\multicolumn{1}{|c|}{Provider}                            & AWS, Azure  & \multicolumn{1}{c|}{CPU (pc.) / RAM (GB)}   & \multicolumn{1}{c|}{1 - 6} \\ \hline
\multicolumn{1}{|c|}{CPU (pc.) / RAM (GB) / Storage (GB)} & 16 - 100    & \multicolumn{1}{c|}{Storage (GB)}           & \multicolumn{1}{c|}{1 - 10} \\ \hline
\multicolumn{1}{|c|}{Idle Power (W)}                      & 150 - 225   & \multicolumn{1}{c|}{Image Size (MB)}        & \multicolumn{1}{c|}{1 - 500} \\ \hline
\multicolumn{1}{|c|}{Max Power (W)}                       & 500 - 3500  & \multicolumn{1}{c|}{Instance (pc.)}         & \multicolumn{1}{c|}{1 - 3} \\ \hline
\multicolumn{1}{|c|}{Bandwidth (Mbps)}                    & 50 - 1200   & \multicolumn{1}{c|}{Message Size (kB)}      & \multicolumn{1}{c|}{2} \\ \hline
\multicolumn{1}{|c|}{Latency (ms)}                        & 15 - 100    &                                             &                       \\ \cline{1-2}
\multicolumn{1}{|c|}{Price (EUR / hour)}                  &  0.025 - 25 &                                             &                       \\ \cline{1-2}
\end{tabular}
}
\end{table}

First, as input, the simulator receives application descriptions in TOSCA-like format, as discussed in Section \ref{sec:application}. This representation accepts two types of application components: \textit{compute} and \textit{storage}. A \textit{compute} unit includes the CPU and memory requirements and also refers to an image file for instantiation. In addition, the number of instances, the provider and the physical location might appear as optional requirements. For a \textit{storage} type, only the size of the allocated partition must be specified, but it can also be restricted to the provider and the location properties. During the evaluation, six application descriptions are submitted to the simulated Swarmchestrate framework with the parameters detailed in Table \ref{tab:params}. The applications are submitted simultaneously to evaluate the response of the system to a wave of deployment requests.

When the application owner submits the application definition, the network randomly selects the RA that will manage the deployment. Each RA is modelled as a lightweight virtualised resource in this environment, utilising 1 CPU core and 1 GB of memory of the underlying physical resource. Therefore, the simulation also requires setting up different nodes, i.e. capacity providers (discussed in Section \ref{sec:resource-agent}). Their configurations are also described in Table \ref{tab:params}, where the current values are selected within the specified interval. Resource-constrained nodes are considered edge devices, moderately powerful nodes are fog resources, and nodes with properties closer to the upper bound are considered cloud nodes. Each RA is deployed on a node, representing and providing the remaining capacity for the application components. 

As soon as each RA receives the application requirements after the broadcast (see Figure \ref{fig:offers}), it performs matchmaking with the application components, attempting to allocate them to its available capacity. In the simulator, this mapping is achieved by first fit search with two variants: each RA either sorts the application components based on their CPU requirements increasing or decreasing. With the ordered list of components, the RAs try to cover as many components as their capacity allows, and to avoid overutilisation, after successful mapping, the related subset of capacity goes into a so-called \textit{reserved} state. 

In the evaluation, half of the RAs use the first fit increasing algorithm, whilst the rest of them execute the first fit decreasing algorithm. This approach helps to avoid a case where only components with higher CPU requirements are mapped to capacities. When RA-X receives all RA - application component pairs (including its own), it creates the offers such that all unique combinations of the pairs are included, with each application component appearing exactly once. Then, for each offer, the QoS attributes (i.e. latency, bandwidth, energy consumption, and pricing) are summed based on the characteristics of the RAs and their capacity participating in the given offer. In case there is no full coverage available, the application request might be resubmitted or rejected. In this paper, we configure the system so that each application can be hosted on Swarmchestrate.

%\begin{figure*}[t]
%    \centering
%    \includegraphics[width=\textwidth]{figures/figure_RAs.jpg}
%    \caption{Resource offer submission and acknowledgment of the resource agents for the deployment}
%    \label{fig:distributed_offers}
%\end{figure*}


\subsection{Resource Selection Methods}\label{sec:ranking}

To rank the all possible combinations of resource offers, and find the optimal resource offer depending on QoS attributes and priorities, we consider two approaches and their variations depending on how they aggregate the reliability scores, as given in Subsections \ref{subsection_cost_func} and \ref{subsection_borda}. 

\subsubsection{\textbf{The Cost Function}}
\label{subsection_cost_func}
%\noindent$\rightarrow$ The cost function and how the best-ranked offer is found should be explained. \\
%$\rightarrow$ Ismail will add a simple equation that outlines the cost function along with some explanation here

In our decentralised resource selection framework, the cost function serves as a core mechanism for evaluating and ranking resource offers based on application-specific Quality of Service (QoS) attributes. The cost-based approach assigns a cost value to each resource offer by normalizing and weighting the QoS attributes according to their priority, as defined by the application. The ranking is then determined by finding the offers with the lowest overall cost.

For each QoS attribute $q \in Q$ (e.g., latency, cost, bandwidth, energy consumption), the raw data $r_q$ is normalized using \eqref{eq:1}.

\begin{align}
\label{eq:1}
\text{\small normalized}_q = \begin{cases} 
\ \ \ \ \ \ \ 0, & \text{\small if \ } \text{\small \textit{max}}(r_q)  = \text{\small \textit{min}}(r_q) \\ 
\frac{r_q - \min(r_q)}{\max(r_q) - \min(r_q)}, & \text{\small otherwise}
\end{cases}
\end{align}

This normalization ensures that each QoS metric is scaled to a comparable range between 0 and 1. For attributes such as bandwidth, where higher values are preferable, the normalized values are inverted to reflect their desirability. The normalized data is then multiplied by the corresponding QoS priority weight $p_q$, specified by the application requirements. The total cost for an offer $i$ is computed in \eqref{eq:2}.


\begin{align}
\label{eq:2}
\text{total\_cost}_i = \sum_{q \in Q}{p_q \cdot \text{normalized}_{q,i}}
\end{align}

Two variants of the cost-based approach integrate reliability scores $R$, which reflect the likelihood of a resource fulfilling its advertised performance:


\textbf{Additive Approach} The reliability is subtracted from the total cost, reducing the cost for more reliable offers. The adjusted cost in this case, $\text{additive\_cost}_i$, can be expresses as $\text{total\_cost}_i - R_i$.

\textbf{Multiplicative Approach} The complement of reliability scales the total cost, which makes the $\text{multiplicative\_cost}_i$ equal to $(1-R_i) \cdot \text{total\_cost}_i$.


\subsubsection{\textbf{Borda Voting Method}}
\label{subsection_borda}
%\noindent$\rightarrow$ The voting approach is to be explained here. Ismail is in charge.

The Borda voting method is a voting-based ranking algorithm that assigns scores to resource offers based on their relative positions across multiple Quality of Service (QoS) attributes. Each QoS attribute contributes to the final ranking of resource offers according to a specified priority weight.

Without considering reliability, each QoS attribute is sorted independently according to its preference, e.g., bandwidth in descending order and latency in ascending order. A Borda count assigns scores based on rank, with the highest-ranked offer receiving the largest score and ties sharing the highest score for their rank. Scores are then weighted by the attribute's priority, summed across all QoS attributes, and used to rank offers. \eqref{eq:3} defines the final Borda score $S_i$ of offer $i$, where $\text{score}_{q}(i)$ and $\text{score}_{R}(i)$ represent the Borda scores for QoS attribute $q$ and reliability $R$, respectively.

\begin{align}
\label{eq:3}
S_i = \sum_{q \in Q}{p_q \cdot \text{score}_{q}(i)}
\end{align}

Similar to the cost function approach, the Borda approach can also incorporate reliability into the evaluation process, either as an additive or multiplicative factor. The final Borda scores with reliability as additive and multiplicative factors are given in \eqref{eq:4} and \eqref{eq:5}, respectively. 

\begin{align}
\label{eq:4}
S_i = \text{score}_{R}(i) + \sum_{q \in Q}{p_q \cdot \text{score}_{q}(i)}
\end{align}

\begin{align}
\label{eq:5}
S_i = R_i \sum_{q \in Q}{p_q \cdot \text{score}_{q}(i)}
\end{align}


\subsection{Application deployment}

After selecting the winning group of RA - application component pairs, the broadcasting (similarly to Figure \ref{fig:leadresource}) has to be repeated because the previously reserved capacity must be reset to \textit{free} if it does not belong to the winning offer, so it can be reused for the following application request later; otherwise, it is set to \textit{assigned}. 

The final step of RA-X is to identify and initialise the deployment of the LR (see Figure \ref{fig:leadresource}). Currently, it is achieved by looking for the components that utilises the most CPU cores. Once its deployment is completed, it triggers the rest of the application components to be deployed as well. When a component is running, the status of its underlying capacity will be modified to be \textit{allocated}. Although the primary goal of this paper and its implementation is to mimic the deployment phase, we also emphasize the long-term impact of this deployment decision by submitting a 30-minute task that fully utilizes the CPU cores of each deployed \textit{compute} component. This step also presents the realisation of post-deployment presented in Figure \ref{fig:post-deployment}.


\subsection{Results}

\begin{table*}[ht!]
\centering
\caption{Simulation results for different priorities and resource selection methods}
\label{tab:res}
\begin{tabular}{|cc|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{Priority}                                          & Method & Simulation Time (min)          & Total Price (EUR)             & Avg. Deployment Time (min)    & Total Energy (KWh)            \\ \hline\hline
\rowcolor[HTML]{E2E2E2} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{E2E2E2}}                          & Borda  & \cellcolor[HTML]{E6B8AF}37.946 & 0.053                         & 3.636                         & 2.232                         \\ \cline{2-6} 
\rowcolor[HTML]{E2E2E2} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{E2E2E2}Energy}}  & Cost   & \cellcolor[HTML]{E6B8AF}37.946 & 0.046                         & \cellcolor[HTML]{E6B8AF}3.779 & \cellcolor[HTML]{B6D7A8}2.170 \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}}                          & Borda  & 35.044                         & \cellcolor[HTML]{B6D7A8}0.015 & 2.451                         & 2.292                         \\ \cline{2-6} 
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Price}}   & Cost   & 37.946                         & 0.032                         & 3.645                         & 2.211                         \\ \hline
\rowcolor[HTML]{E2E2E2} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{E2E2E2}}                          & Borda  & 34.641                         & 0.077                         & 1.352                         & 2.360                         \\ \cline{2-6} 
\rowcolor[HTML]{E2E2E2} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{E2E2E2}Latency}} & Cost   & 34.562                         & 0.079                         & 1.285                         & \cellcolor[HTML]{E6B8AF}2.363 \\ \hline
\multicolumn{1}{|c|}{}                                                  & Borda  & \cellcolor[HTML]{FFFFFF}34.385 & \cellcolor[HTML]{FFFFFF}0.075 & \cellcolor[HTML]{FFFFFF}1.288 & \cellcolor[HTML]{FFFFFF}2.316 \\ \cline{2-6} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{Bandwidth}}                       & Cost   & \cellcolor[HTML]{B6D7A8}32.175 & \cellcolor[HTML]{E6B8AF}0.115 & \cellcolor[HTML]{B6D7A8}0.968 & \cellcolor[HTML]{FFFFFF}2.260 \\ \hline
\rowcolor[HTML]{E2E2E2} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{E2E2E2}}                          & Borda  & 34.318                         & 0.036                         & 1.620                         & 2.229                         \\ \cline{2-6} 
\rowcolor[HTML]{E2E2E2} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{E2E2E2}Equal}}   & Cost   & 34.562                         & 0.076                         & 1.285                         & \cellcolor[HTML]{E6B8AF}2.363 \\ \hline
\multicolumn{2}{|c|}{Random}                                                     & 34.437                         & 0.082                         & 1.365                         & 2.310                         \\ \hline
\end{tabular}
\end{table*}

\begin{figure*}[ht]
    \centering
    \includesvg[width=0.49\textwidth]{figures/energy-prior-chart.svg} \hfill
    \includesvg[width=0.49\textwidth]{figures/latency-prior-chart.svg}
    \caption{Energy consumption per node with energy priority (left) and latency priority (right)}\label{fig:res}
\end{figure*}

To simulate the Swarmchestrate framework in a realistic manner, we also set up an image registry (e.g., Docker Hub) with 1000 Mbps bandwidth in the DISSECT-CF-Fog simulator. The aim of this service is to store the image files of the application components. Once the winning group of RAs with the capacity reservations are determined, the image files are transferred over the network where the actual application component has to be deployed. The simulator also measures the energy consumption that occurs during network communications and CPU usages.

During the evaluation, we examined how the framework handles the simultaneously submitted six application when the focus is on the different priority values of the QoS attributes. In addition to the randomly selected offer, we employed five other strategies: one where all priorities were equal, and another where one of the four priorities was set to 1.0 while the remaining three were set to 0.1. The results are presented in Table \ref{tab:res}. The application submission are managed by eight fully connected RAs and their associated capacities provided by eight nodes.

For comparison, we took into account the following metrics: (i) \textit{Simulation Time} measures the time needed from the first application submission to the completion of the last CPU-intensive task performed. (ii) \textit{Total Price} follows the pay-as-you-go pricing schema based on the hourly usage price of the RA. (iii) \textit{Avg. Deployment Time} focuses only on the application deployment phase, measuring the time interval between the submission of the application and the deployment of its components, which is mainly influenced by the latency and bandwidth properties. Lastly, (iv) \textit{Total Energy} shows the aggregated energy consumed by the nodes during the \textit{Simulation Time}. 

Table \ref{tab:res} depicts the best values with green background colour and the worst values with red background colour for each metric, demonstrating how the Borda and Cost approaches perform. It can be seen that in the cases (row 1-8) where a priority value of 1.0 was set, the proposed ranking algorithm effectively selected the group of RAs compared to other strategies (green columns). For instance, if the application owner priorities money saving, it can be achieved by choosing the price-aware strategy. 

It is also notable that the Cost method generally outperforms the Borda method in finding the best value according to priority, but the worst values (red columns) also belong to the Cost ranking. To counterbalance this behaviour, the Equal method reveals a trade-off between cost and deployment efficiency. It is also worth noting that prioritizing latency alone does not optimise the application deployment time as effectively as the bandwidth-aware approach.We can conclude that bandwidth plays a decisive role in the application deployment process.

To provide further insight into the simulation, more specifically the energy usage, Figure \ref{fig:res} shows the energy consumption per node when executing the energy and latency-aware approaches. The simulation, including the setup of edge, fog, and cloud resources and the associated RAs, starts from scratch, thus the figure only presents the energy consumed after the applications were submitted. This means that energy was accumulated during only the broadcast messaging, the deployment of the application component, and the execution of CPU-heavy tasks. The latter consumes significantly more energy, which can be observed in both subfigures: in the case of the energy-aware approach, the CPU-heavy tasks start after the fifth minute, while the latency-aware strategy results in faster application deployment (as it is shown by \textit{Avg. Deployment Time} in Table \ref{tab:res} as well), thus related tasks already start after the third minute.

==> problem.tex <==
\section{Problem definition \textcolor{blue}{(Amjad/Tamas/Ismail)}}
\noindent$\rightarrow$ Discuss the problem within the context of multiple resource providers \\
\noindent$\rightarrow$ Then raise the questions, how the application can be submitted, the resource offers collection, optimal resource selection, Swarm formation, and self-organization \\

==> swarmchestrate_copy.tex <==
\section{Swarmchestrate: Proposed approach \textcolor{blue}{(Amjad/Tamas/Ismail/Andras)}}
%\noindent$\rightarrow$ Present architecture, discuss the concept with a brief description of the Application view, Resource view and Knowledge Mgmt and a strong emphasis on Orchestration Space covering all processes: \\
%\indent $\rightarrow$ Resource offers collection \\
%\indent $\rightarrow$ Resource selection \\
%\indent $\rightarrow$ Lead SA deployment \\
%\indent $\rightarrow$ Application deployment \\ 
\textcolor{blue}{Status: In progress and will change soon}\\
\begin{figure*}[t]
    \centering
        \includegraphics[width=0.9\textwidth]{figures/framework.png}
        \caption{Swarmchestrat architecture}
        \label{fig:framework}
\end{figure*}
Figure~\ref{fig:framework} illustrates the architectural view of the Swarmchestrate application deployment process. The overall system is organised into four key sections. \textbf{Application view} enables application operators to define their applications using the standardized TOSCA application description format~\textcolor{blue}{Cite here}. It focuses on four essential aspects: the specification of application microservices, resource requirements, monitoring parameters, and desired Quality of Service (QoS) objectives. The \textbf{Resource view} consists of a two-layered approach, where \textit{Resources} represents the actual computational resources provided by different cloud and edge providers, e.g. Amazon, Microsoft, etc., and \textit{Capacity}, refers to the logical grouping of resources offered (made available) by an entity within the Swarmchestrate ecosystem. Thus, any resource in the Swarmchestrate is part of a capacity, which must be registered through the Knowledge Management to be discovered and utilized for application deployment.

The \textbf{Knowledge Management} component serves as a distributed knowledge base, handling information related to resource capabilities, their descriptions, system interactions, and decision-making processes. Resources can be discovered based on diverse contextual attributes and trust factors, facilitating efficient application deployment and dynamic reconfiguration.
Lastly, the \textbf{Orchestration Space (OS)} is a decentralised entity with no central control point, serving as the execution environment for key orchestration activities. This paper focuses on the OS component, emphasising the application deployment stage. The remainder of this section provides detailed insights into this aspect.

OS is the confluence of three key concepts---decentralisation, swarms, and intelligence---for achieving efficient, optimized, and trusted application orchestration in the Cloud-Edge ecosystem. The notion of decentralisation is due to its adopted distributed architecture; swarm is the adaptation of the swarm computing concept for executing and managing individual applications as swarms; and intelligence is its strong reliance on the use of machine learning and optimisation-based algorithms for resource selection and reconfigurations decision-making. The following sub-sections explain the various parts of the OS.

\subsection{Application}\label{sec:application}
Swarmchestrate focuses on microservices-based applications rather than monolithic ones, with each application consisting of $m$ distinct components such as $app = \{comp_1, comp_2, \dots, comp_m\}$. The type of each component can be either compute or storage: $type_{comp_i} \in \{compute, storage\}, \quad \forall i \in \{1, 2, \dots, m\}$, where each has a set of resource requirements, $req_{comp_i} = \{req_1, req_2, \dots, req_k\}$. The resource requirements can be of two forms: Mandatory ($req_{mandatory, comp_i}$), and optional ($req_{optional, comp_i}$). The mandatory resource requirements for each component vary based on its type. For compute components, these requirements include the number of CPU cores, memory capacity, and an image file necessary for resource instantiation. For storage components, the specified requirements include the size of the allocated storage partition. Thus:

\[
\small
req_{mandatory, comp_i} =
\begin{cases}
\langle cpu, memory, image \rangle & \\\indent  \text{if } type_{comp_i}=compute \\
\langle size \rangle & \\\indent \text{if } type_{comp_i}=storage \\
\end{cases}
\]

Optional parameters, such as the number of application instances for compute components, the provider specification (e.g., AWS), and the service's geographical location (e.g., Europe), must also be defined. Formally:

\[
req_{optional, comp_i} =
\begin{cases}
\langle instances, provider, location \rangle & \\\indent \text{if }  type_{comp_i} = compute \\
\langle provider, location \rangle & \\\indent \text{if } type_{comp_i} = storage \\
\end{cases}
\]

As mentioned earlier, the application in Swarmchestrate will be described in TOSCA format. This description is submitted to the OS interface, a network of Resource Agents (RAs). The next section explains the role of RAs and the process.
\subsection{Resource Agent (RA)}
The RA is the key system component responsible for providing access to the resources of a capacity. In collaboration with other RAs, it also facilitates the discovery of suitable resources for submitted applications. More formally, in the Swarmchestrate framework, there are multiple resource agents, $ ra = \{ ra_1, ra_2, \dots, ra_n \} $, where $n$ represents the total number of RAs in the orchestration space. They operate independently, however, connected within a P2P network, functioning without a central entity. 

Each $ra_i$ has the following attributes: (i) a host (i.e., edge or cloud node) $host_{ra_i}$, where the resource agent service resides; (ii) a capacity set $cap_{ra_i}$, where each $cap_j$ of the capacity set $cap= \{ cap_1, cap_2, \dots, cap_l \}$ represents the available CPU cores, memory, and storage size for the particular $ra_i$; (iii) $price_{ra_i}$, specifying the unit cost of utilizing the resources managed by the resource agent; and (iv) a strategy $strat_{ra_i}$ that indicates the decision-making logic for offering capacity resources for various application components. Thus:

\[
ra_i = \langle node, cap, price, strat \rangle
\]

Upon an application's arrival, the receiving RA triggers its overall deployment process, which is explained in the next section.

\subsection{Overall deployment process}\label{sec:appDeployment}
\paragraph{Collecting resource offers}
\paragraph{Resource selection}
\paragraph{Lead SA deployment}
\paragraph{Application deployment}




\subsection{Formal Description of the Application}

The Swarmchestrate framework can receive applications at any point in its lifetime to be deployed on its architecture. In this work, an application consists of microservices instead of considering monolithic applications. Let $app$ denote such an application consisting of $m$ components: $app = \{comp_1, comp_2, \dots, comp_m\}$. Each component can take one of two values, formally:

\[
type_{comp_i} \in \{compute, storage\}, \quad \forall i \in \{1, 2, \dots, m\}.
\]

Each component has a set of resource requirements, $req_{comp_i} = \{req_1, req_2, \dots, req_k\}$, which are divided into two groups. The first group represents mandatory resource requirements, denoted as $req_{mandatory, comp_i}$, and the second group represents optional resource requirements, denoted as $req_{optional, comp_i}$. Thus:

\[
req_{comp_i} = req_{mandatory, comp_i} \cup req_{optional, comp_i}
\]

and

\[
req_{mandatory, comp_i} \cap req_{optional, comp_i} = \emptyset.
\]

The mandatory resource requirements for each component depend on the type of the component. For a compute type, this includes the number of CPU cores, memory requirements, and an image file needed for initializing the virtual resources. For a storage type, the storage size of the allocated partition must be specified. Thus:

\[
\small
req_{mandatory, comp_i} =
\begin{cases}
\langle cpu, memory, image \rangle & \\\indent  \text{if } type_{comp_i}=compute \\
\langle size \rangle & \\\indent \text{if } type_{comp_i}=storage \\
\end{cases}
\]

Optional parameters, such as the number of application instances for compute components, the provider specification (e.g., AWS), and the service's geographical location (e.g., Europe), must also be defined. Formally:

\[
req_{optional, comp_i} =
\begin{cases}
\langle instances, provider, location \rangle & \\\indent \text{if }  type_{comp_i} = compute \\
\langle provider, location \rangle & \\\indent \text{if } type_{comp_i} = storage \\
\end{cases}
\]

When the application owner submits the application definition to the Swarmchestrate framework, the network randomly selects the resource agent (detailed in the next section) that will manage the deployment. This approach is advantageous due to its simplicity. However, in the future, we will also explore more sophisticated solutions, such as proximity-based selection or gossip protocol-based approach.  

\subsection{Formal Specification of Resource Agent}

The key system component when an application is submitted is the resource agent. It is considered a lightweight service designed to grant access to the resources of a specific capacity provider. In the Swarmchestrate framework, multiple resource agents, $ ra = \{ ra_1, ra_2, \dots, ra_n \} $, where $n$ is the total number of available resource agents in the orchestration space, operate within a fully connected network, functioning without a central entity. Each $ra_i$ is hosted by one of the nodes, $node = \{node_1, node_2, \dots, node_v\}$, which are also responsible for hosting the components of the applications. Each node has a geographical location and depending on its constraints, they can be either edge devices, fog nodes or cloud providers.

Each $ra_i$ has the following attributes: (i) a host (i.e., edge or cloud node) $host_{ra_i}$, where the resource agent service resides; (ii) a capacity set $cap_{ra_i}$, defining the logical grouping of resources offered by a provider (e.g., AWS); (iii) $price_{ra_i}$, specifying the unit cost of utilizing the resources managed by the resource agent; and (iv) a strategy $strat_{ra_i}$ that indicates the decision-making logic for offering capacities for various application components. Thus:

\[
ra_i = \langle node, cap, price, strat \rangle
\]

Furthermore, each $cap_j$ of the capacity set $cap= \{ cap_1, cap_2, \dots, cap_l \}$ represents the available CPU cores, memory, and storage size for the particular $ra_i$. These capacities might be from various hosts, and the current state of the capacity can take one of the following values: (i) \textit{free}, meaning the capacity is unused and available to be utilized by an application component; (ii) \textit{reserved}, meaning the given capacity is offered for utilization but the decision has not yet been made; (iii) \textit{assigned}, meaning the capacity was chosen but deployment has started and is not yet finished; and (iv) \textit{allocated}, meaning the capacity is under utilization by an application component. Therefore, the fifth attribute denotes the application component that is considered to be utilised by the given application component. This parameter is set only when the state equals \textit{reserved}, \textit{assigned}, or \textit{allocated}.

\[
cap_j = \langle cpu, memory, size, state, comp_i \rangle
\]

and

\[
state \in \{free, reserved, assigned, allocated \}.
\]


\begin{algorithm*}
\caption{Gateway Selection and Requesting Offers}
\label{alg:gateway}

\KwIn{$ra = \{ra_1, ra_2, \dots, ra_n\}$, the set of resource agents}
\KwIn{$app = \{comp_1, comp_2, \dots, comp_m\}$, the application components}
\KwOut{$OfferCollection$, a collection of $(ra_i, comp_j)$ pairs}

$OfferCollection \gets \emptyset$ \\
$ra_{gateway} \gets \text{Select}(ra)$ \\

\BlankLine
\textbf{\textit{@parallel}} \\
\ForEach{$ra_i \in ra \setminus \{ra_{gateway}\}$}{
    $ra_{gateway}$ sends $message(app)$ to $ra_i$ \\
    $offers_{ra_i} \gets strat_{ra_i}(app)$ \\
    $ra_i$ sends $message(offers_{ra_i})$ back to $ra_{gateway}$ \\
    $OfferCollection \gets OfferCollection \cup offers_{ra_i}$
}

\KwRet{$OfferCollection$}
\end{algorithm*}


\begin{algorithm*}
\caption{First Fit Algorithm for Resource Allocation}
\label{alg:firstfit}

\KwIn{$ra_i$, a resource agent with a set of capacities $cap_{ra_i}$}
\KwIn{$app = \{ comp_1, comp_2, \dots, comp_m \}$, the application components}
\KwOut{$Offers$, a set of $(ra_i, comp_j)$ pairs}

$Offers \gets \emptyset$ \\
$SortedComponents \gets SortByCpuThenSize(app, flag)$ \\

\ForEach{$comp_j \in SortedComponents$}{
    \uIf{$type_{comp_j} = compute$}{
        $NumOfInstances \gets req_{comp_j}(instances)$ \\
        $Requirements \gets req_{comp_j}(cpu, memory, location, provider)$ \\
        
        $ReservedCapacities \gets \emptyset$ \\
        
        \For{$i \gets 1$ \KwTo $NumOfInstances$}{
            \ForEach{$cap_j \in ra_i.cap$ \textnormal{ where } $cap_j.state = free$}{
                \If{$cap_j \textnormal{ satisfies } Requirements$}{         
                 % $Requirements \subseteq cap_j \quad \Rightarrow \quad cap_j.state \gets reserved$ \\
                    $cap_{new} \leftarrow \langle cpu, memory, size, reserved, comp_i \rangle$ \\
                    $cap_j \leftarrow cap_j - cap_{new}$ \\
                    $ReservedCapacities \gets ReservedCapacities \cup cap_{new}$ \\
                    \textbf{break}
                }
            }
        }

        \uIf{$NumOfInstances = |ReservedCapacities|$}{
            $ra_i.cap \leftarrow ra_i.cap \cup ReservedCapacities$ \\
            $Offers \gets Offers \cup \{(ra_i, comp_j)\}$ \\
        }
        \Else{
            \ForEach{$cap_j \in ReservedCapacities$}{
                $cap_{used} \leftarrow cap_{used} + cap_{j}$ \\
                $cap_j.state \gets free$ \\
            }
        }
    }
    \ElseIf{$type_{comp_j} = storage$}{
        $Requirements \gets req_{comp_j}(size, location, provider)$ \\
        \ForEach{$cap_j \in ra_i.cap$}{
            \If{$cap_j \textnormal{ satisfies } Requirements$}{               
                $Requirements \subseteq cap_j \quad \Rightarrow \quad cap_j.state \gets reserved$ \\
                $Offers \gets Offers \cup \{(ra_i, comp_j)\}$ \\
            }
        }
    }
}

\Return{$Offers$}
\end{algorithm*}


\subsection{Combination of Offers}

\begin{algorithm*}
\caption{Generate Unique Combinations of the Collection of Offers}
\label{alg:generate_combinations}
\KwIn{$pairs$, a collection of $(ra_i, comp_j)$ pairs}
\KwIn{$componentCount$, the count of the components in $app$}
\KwOut{$uniqueCombinations$: A set of all unique combinations of pairs $(ra_i, comp_j)$ such that each combination includes exactly $componentCount$ components}

\BlankLine
\textbf{Main Procedure:}\\

$uniqueCombinations \gets \emptyset$ \\
$currentCombination \gets \emptyset$ \\
$includedComponents \gets \emptyset$ \\

GenerateCombinations($pairs$, $componentCount$, $uniqueCombinations$, $currentCombination$, $includedComponents$) \\

\BlankLine
\textbf{GenerateCombinations(...) Procedure:} \\
    \If{$|includedComponents| = componentCount$}{
        Add $currentCombination$ to $uniqueCombinations$ \\
        \textbf{return}\ \\
    }

    \ForEach{$(ra_i, comp_j) \in pairs$}{
        \If{$(ra_i, comp_j) \notin currentCombination$ \textbf{and} $comp_j \notin includedComponents$}{
            Add $(ra_i, comp_j)$ to $currentCombination$ \\
            Add $comp_j$ to $includedComponents$ \\
            GenerateCombinations(...) \\
            Remove $(ra_i, comp_j)$ from $currentCombination$ \\
            Remove $comp_j$ from $includedComponents$ \\
        }
    }
\end{algorithm*}
